NP-DRAW: A Non-Parametric Structured Latent Variable Model for Image Generation

In this paper, we present a non-parametric structured latent variable model for image generation, called NP-DRAW, which sequentially draws on a latent canvas in a part-by-part fashion and then decodes the image from the canvas. Our key contributions are as follows. 1) We propose a non-parametric prior distribution over the appearance of image parts so that the latent variable ``what-to-draw'' per step becomes a categorical random variable. This improves the expressiveness and greatly eases the learning compared to Gaussians used in the literature. 2) We model the sequential dependency structure of parts via a Transformer, which is more powerful and easier to train compared to RNNs used in the literature. 3) We propose an effective heuristic parsing algorithm to pre-train the prior. Experiments on MNIST, Omniglot, CIFAR-10, and CelebA show that our method significantly outperforms previous structured image models like DRAW and AIR and is competitive to other generic generative models. Moreover, we show that our model's inherent compositionality and interpretability bring significant benefits in the low-data learning regime and latent space editing. Code is available at https://github.com/ZENGXH/NPDRAW.

==> others.tex <==

\subsection{Other Evaluation Tasks in Related Work}

\subsubsection{Unsupervised Classification}
The SCAE paper perform unsupervised classification (also called unsupervised class discovery in images) on three dataset: MNIST, SVHN, CIFAR10. It compared to mutual information based method. Two classifier based on the SCAE model is proposed: 
\begin{enumerate}
    \item LIN-MATCH: clustering into 10 clusters (kmeans) + bipartite graph matching to find the permutation of cluster indices that minimizes the classification error—this is standard practice in unsupervised classification,
    \item LIN-PRED: train a linear classifier without changing weight of the main model 
\end{enumerate}

\subsubsection{Cluttered MNIST Classification To Test the Attention Mechanism}
Used in the DRAW paper.

\subsubsection{Counting}
Used in AIR paper, count the Multi-MNIST dataset. AIR paper also test the generalization ability by training AIR model on images with K digits and testing it on non-K digits. 

\subsubsection{Representational Power}
Used in AIR paper, we split
this data into training and test and consider two
tasks: (a) predicting the sum of the two digits, and (b) determining if the
digits appear in an ascending order.

\subsubsection{Others}
1) AIR paper also works with 3D scene. 2) VQVAE test the generalization on audio, and video. 

\section{More Details for Related Works}
\subsection{Part Capsule Auto-encoder (PCAE)} \label{sec:pcae} 
\textbf{More details} For the $m^{th}$ capsule, the encoder predict $r_m \in \mathbb{R}^6$ ( rotation, translation, scale, shear) and presence $d_m \in [0, 1]$, the decoder predict the template $T_m=T_m^{alpha}, T_m^c$. For MNIST, they set the size of template is $11\times11$ and number of capsules  $M=24$. The image likelihood $ p(x) $ can be written as 
\begin{equation}
    p(x) = \prod_{i, j} \sum_{m}^M \underbrace{(d_m \hat{T}_{m, i, j}^{alpha})}_{\text{mixing prob}} \mathcal{N}(y_{i, j}| \hat{T}_{m,i,j}^c; \sigma_y^2),
\end{equation}
where $\hat{T}_m = \text{TransformImage}(T_m, r_m)$. The model is optimized by MLE. The key is the design of using $r_m$ to transform $T_m$, which forces the model to learn the structure. The paper reports unsupervised classification performance.  

\subsection{Human Concept Learning} \label{sec:hcl} 
The generation process can be viewed in Fig~\ref{fig:bpl}. In their cases, the primitives set is extracted from the Omniglot dataset. They first break every strokes in the dataset into sub-strokes (55,000), according to the time pause threshold, and then perform GMM to create the primitives set (size 1250). Given the breaking procedure, most of the distribution can be directly estimated on the training dataset. The paper reports performance on one-shot learning. 

There are two main stages for generation, 
\begin{itemize}
    \item generate character type $\varphi = \{\kappa, S, R\}$, where $\kappa$ is number of stroke $S=\{S_1, ..., S_\kappa\}$ and their spatial relation $R=\{R_1, ..., R_\kappa\}$, its joint distribution is written at the bottom of Fig~\ref{fig:bpl}. For each stroke $S_i=\{s_{i}^1, ... , s_{i}^{n_i}\}$, need to generate its template trajectory (a sequence of sub-strokes $\{z_i^j\}$: type $z_{i}^j$ and scale). $P(\varphi) = p(\kappa) \prod_i^\kappa P(S_i)P(R_i|S_{<i})$, $R\in$ \{independent, start, end, along\}. 
    \item generate the raw image given the character $\varphi$, where some random transformation will be performed to create variant images. $P(I|\varphi, \theta_{trans})$
\end{itemize}

\textit{Empirical distribution directly:} number of strokes $p(\kappa)$, number of sub-parts $p(n_i | \kappa)$, transition of the primitive type $z_{i}^j \in \{1,..,1250\}$, $z_{i}^j \sim p(z_{i}^j | z_{i}^{j-1})$. 

\textit{Estimated by fitting the motor program:} 1) the probabilities of different relationship type $\theta_R$, and 2) the token-level (image-level) variance for shape, scale and attachment variables. 

\begin{itemize}
\item [+] can be used for one-shot learning: the fitted program is able to generate variant of the same object 
\item [-] The produce is too hand-crafted. 
\end{itemize}

\paragraph{Task setup}
Three tasks are proposed to evaluate one-shot generalization~\cite{lake2015human,DBLP:conf/icml/RezendeMDGW16}, from easy to hard: 
\begin{enumerate}
    \item unconditional (free) generation
    \item generation of novel variations of a given exemplar
    \item generation of representative samples from a novel alphabet
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibliography{example_paper}
\bibliographystyle{icml2019}

==> tbl_architecture.tex <==

\begin{table}[h]
  \scriptsize
  \setlength{\tabcolsep}{5pt}
\begin{sc}
   \begin{tabular}{c p{0.27\linewidth} p{0.27\linewidth} p{0.27\linewidth}}
       & MNIST & CIFAR\_10 & CELEBA \\
       \toprule
       Encoder: &
       $x \in \mathcal{R}^{32{\times}32}$ \newline
       $\rightarrow \text{Conv}_{128} \rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{1024}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Flatten} \rightarrow \text{FC}_{16{\times}M}$
     & $x \in \mathcal{R}^{32{\times}32}$ \newline
       $\rightarrow \text{Conv}_{128} \rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{1024}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Flatten} \rightarrow \text{FC}_{128{\times}M}$
     & $x \in \mathcal{R}^{64{\times}64}$ \newline
       $\rightarrow \text{Conv}_{128} \rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Conv}_{1024}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\quad \rightarrow \text{Flatten} \rightarrow \text{FC}_{64{\times}M}$\\

\midrule
Decoder: &
       $z \in \mathcal{R}^{16} \rightarrow \text{FC}_{8{\times}8{\times}1024}$\newline
       $\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{1}$
     & $z \in \mathcal{R}^{128} \rightarrow \text{FC}_{8{\times}8{\times}1024}$\newline
       $\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{1}$
     & $z \in \mathcal{R}^{64} \rightarrow \text{FC}_{8{\times}8{\times}1024}$\newline
       $\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{512}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{256}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{128}\rightarrow \text{BN} \rightarrow \text{ReLU}$\newline
       $\rightarrow \text{ConvT}_{1}$ \\
 \bottomrule
   \end{tabular}
\end{sc}
\end{table}

